Comprehension and quotient structures in the language of 2-categories

Lawvere observed in his celebrated work on hyperdoctrines that the set-theoretic schema of comprehension can be elegantly expressed in the functorial language of categorical logic, as a comprehension structure on the functor $p:\mathscr{E}\to\mathscr{B}$ defining the hyperdoctrine. In this paper, we formulate and study a strictly ordered hierarchy of three notions of comprehension structure on a given functor $p:\mathscr{E}\to\mathscr{B}$, which we call (i) comprehension structure, (ii) comprehension structure with section, and (iii) comprehension structure with image. Our approach is 2-categorical and we thus formulate the three levels of comprehension structure on a general morphism $p:\mathrm{\mathbf{E}}\to\mathrm{\mathbf{B}}$ in a 2-category $\mathscr{K}$. This conceptual point of view on comprehension structures enables us to revisit the work by Fumex, Ghani and Johann on the duality between comprehension structures and quotient structures on a given functor $p:\mathscr{E}\to\mathscr{B}$. In particular, we show how to lift the comprehension and quotient structures on a functor $p:\mathscr{E}\to\mathscr{B}$ to the categories of algebras or coalgebras associated to functors $F_{\mathscr{E}}:\mathscr{E}\to\mathscr{E}$ and $F_{\mathscr{B}}:\mathscr{B}\to\mathscr{B}$ of interest, in order to interpret reasoning by induction and coinduction in the traditional language of categorical logic, formulated in an appropriate 2-categorical way.

==> macros.tex <==

% logic
\newcommand{\infer}[4]{#1\vdash\,#2:#3\;|\;#4}
\newcommand{\infers}[4]{#1\vdash_s\,#2:#3\;|\;#4}
\newcommand{\inferi}[4]{#1\vdash_i\,#2:#3\;|\;#4}
\newcommand{\inference}[2]{\dfrac{#1}{#2}}

\newcommand{\inferencep}[3]{\begin{prooftree}
	\Hypo{#2}
	\Infer1[#1]{#3}
	\end{prooftree} 
}


\newcommand{\catname}[1]{{\normalfont\textbf{#1}}}
%\newcommand{\push}[1]{\text{Push}_{#1}}


\newcommand{\git}{\mathbin{
  \mathchoice{/\mkern-6mu/}% \displaystyle
    {/\mkern-6mu/}% \textstyle
    {/\mkern-5mu/}% \scriptstyle
    {/\mkern-5mu/}}}% \scriptscriptstyle
    
\newcommand{\LaxOver}[2]{#1\git #2} % style1
\newcommand{\varOne}{{-}}
\newcommand{\varTwo}{{=}}
\newcommand{\varThree}{{\equiv}}

%FIXME : devrait etre llbracket
\newcommand{\LaxHomTwoCat}[2]{\llbracket {#1}, {#2} \rrbracket}
%\newcommand{\LaxHomTwoCat}[2]{[#1,#2]}

\newcommand{\comp}[1]{\{{#1}\}}
\newcommand{\rotateit}[1]{\raisebox{\depth}{\rotatebox{180}{#1}}}
\newcommand{\invu}{n}


%\newcommand{\sectiono}[1]{\ast_{#1}}
%\newcommand{\sectiono}[1]{\diamond_{#1}}
\newcommand{\sectiono}[1]{\smallstar_{#1}}
\newcommand{\sectionp}[1]{\smallstar_{#1}}
%\newcommand{\sectionq}[1]{\thinstar_{#1}}
\newcommand{\sectionq}[1]{\ostar_{#1}}
%\newcommand{\sectionr}[1]{\pentagram_{#1}}
%\newcommand{\sectionr}[1]{\diamonddot{#1}}
\newcommand{\sectionr}[1]{\smalldiamond_{#1}}
\newcommand{\sectionid}{i}

\newcommand{\pushstructureid}{(\cod,\sectionid,id, (id,\_),(id,\_),(\_,id))}
%%% styles for PUSH

\newcommand{\push}[2]{\exists_{#1}{[\sectionp{#2}]}} % style1
\newcommand{\pushp}[2]{\exists_{#1}{[\sectionp{#2}]}}
\newcommand{\pushprime}[2]{\exists'_{#1}{[\sectionp{#2}]}} % style1
%\newcommand{\push}[2]{\mathsf{push}_{#1}{[\sectiono{#2}]}} % style2
%\newcommand{\pushabr}[1]{\sectionpushed{#1}} % style2

\newcommand{\pushid}[2]{\exists_{#1}{[id_{#2}]}}
\newcommand{\pushq}[2]{\exists_{#1}{[\sectionq{#2}]}} % style1
%\newcommand{\pushqabr}[1]{\pushq{#1}{}}              % style1
\newcommand{\pushr}[2]{\exists_{#1}{[\sectionr{#2}]}}

% ancienne syntaxe, redirige vers le style choisi
\newcommand{\sectionpushed}[2]{\push{#2}{#1}} % style1
%\newcommand{\sectionpushed}[2]{\ast_{#1}[#2]} % style2

\newcommand{\RHD}{\triangleright}
\newcommand{\LHD}{\triangleleft}

%\newcommand{\pushr}[2]{\exists_{#2}{[\ast{#1}]}}
%\newcommand{\post}[1]{{#1}_{\bullet}}
%\newcommand{\pre}[1]{{#1}^{\bullet}}
%\newcommand{\post}[1]{\langle{#1}|}
%\newcommand{\pre}[1]{|{#1}\rangle}
\newcommand{\postComp}[1]{{#1}^\star}
\newcommand{\preComp}[1]{{#1}_\star}
\newcommand{\postp}[1]{#1{\RHD}}
\newcommand{\prep}[1]{{\LHD}{#1}}
\newcommand{\postq}[1]{#1{\rhd}}
\newcommand{\preq}[1]{{\lhd}{#1}}
\newcommand{\postr}[1]{#1{\smalltriangleright}}
\newcommand{\prer}[1]{{\smalltriangleleft}{#1}}
\newcommand{\postid}[1]{#1{\smalltriangleright}}
\newcommand{\preid}[1]{{\smalltriangleleft}{#1}}

\newcommand{\unitPush}[1]{\lambda_{id_{#1}}}
\newcommand{\unitIdPush}[1]{\lambda_{#1}}
\newcommand{\Pushmap}[1]{\lambda_{#1}}
\newcommand{\Pushmapid}[2]{(id_{#1}, #2)}
\newcommand{\Pushmapp}[1]{\lambda^{\sectionp{}}_{#1}}
\newcommand{\Pushmappprime}[1]{\lambda'^{\sectionp{}}_{#1}}
\newcommand{\Pushmapq}[1]{\lambda^{\sectionq{}}_{#1}}
\newcommand{\Pushmapr}[1]{\lambda^{\sectionr{}}_{#1}}


\newcommand{\Pullmap}[1]{\rho_{#1}}
\newcommand{\homcat}[2]{[#1,#2]}
\newcommand{\dom}{dom}
\newcommand{\cod}{cod}
\newcommand{\ConstArr}{\sectionid}

\newcommand{\Hletter}{H}

\newcommand{\FPrime}{F'}
\newcommand{\FOnly}{F}
\newcommand{\GPrime}{G'}
\newcommand{\GOnly}{G}
\newcommand{\HPrime}{H'}
\newcommand{\HOnly}{H}
\newcommand{\RPrime}{R'}
\newcommand{\ROnly}{R}
\newcommand{\SPrime}{S'}
\newcommand{\SOnly}{S}

\newcommand{\LPrime}{L'}
\newcommand{\LOnly}{L}

\newcommand{\Gprime}{\GPrime}
\newcommand{\Fprime}{\FPrime}
\newcommand{\Hprime}{\HPrime}
\newcommand{\alphaPrime}{\alpha'}
\newcommand{\betaPrime}{\beta'}
\newcommand{\thetaFFprime}{\alpha}
\newcommand{\thetaGGprime}{\beta}

\newcommand\todo[1]{\textcolor{red}{\ifstrempty{#1}{todo}{#1}}}
% various
\newcommand{\underCheck}{\underaccent{\check}}
\newcommand{\underWideCheck}[1]{%
  \mathpalette\doUnderWhideCheck{#1}%
}
\makeatletter
\newcommand{\doUnderWhideCheck}[2]{%
  \sbox0{$\m@th#1\widehat{\hphantom{#2}}$}%
  \sbox2{$\m@th#1x$}
  \sbox4{$\m@th#1#2$}
  \dimen0=\ht0
  \advance\dimen0 -.8\ht2
  \dimen2=\dp4
  \rlap{%
    \raisebox{\dimexpr\dimen0-\dimen2}{%
      \scalebox{1}[-1]{\box0}%
    }%
  }%
  {#2}%
}
\makeatother

\newcommand{\underHat}{\underaccent{\hat}}
\newcommand{\underWideHat}[1]{%
  \mathpalette\doUnderWhideHat{#1}%
}
\makeatletter
\newcommand{\doUnderWhideHat}[2]{%
  \sbox0{$\m@th#1\reallywidecheck{\hphantom{#2}}$}%
  \sbox2{$\m@th#1x$}
  \sbox4{$\m@th#1#2$}
  \dimen0=\ht0
  \advance\dimen0 -.8\ht2
  \dimen2=\dp4
  \rlap{%
    \raisebox{\dimexpr\dimen0-\dimen2}{%
      \scalebox{1}[-1]{\box0}%
    }%
  }%
  {#2}%
}


\newcommand\reallywidehat[1]{%
	\savestack{\tmpbox}{\stretchto{%
			\scaleto{%
				\scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
				{\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
			}{\textheight}% 
		}{0.5ex}}%
	\stackon[1pt]{#1}{\tmpbox}%
}


\makeatother
\newsavebox{\accentbox}
\newcommand{\compositeaccents}[2]{%
  \sbox\accentbox{$#2$}#1{\usebox\accentbox}}

\newcommand{\preLeft}[1]{\hat{#1}}
\newcommand{\preRight}[1]{\check{#1}}
\newcommand{\postLeft}[1]{\underCheck{#1}}
\newcommand{\postRight}[1]{\underHat{#1}}

\newcommand{\preLeftW}[1]{\reallywidehat{#1}}
\newcommand{\preRightW}[1]{\reallywidecheck{#1}}
\newcommand{\postLeftW}[1]{\underWideCheck{#1}}
\newcommand{\postRightW}[1]{\underWideHat{#1}}

\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{\protect\leavevmode\begingroup\color#1{#2}#3\endgroup }

\newcommand{\air}{\medbreak\noindent}
% \renewcommand{\above}[0]{\sqsubset}
\newcommand{\catAdj}{\catname{Adj}}
\newcommand{\catSet}{\catname{Set}}
%\newcommand{\Set}{\catname{Set}}
%\newcommand{\Rel}{\catname{Rel}}
\newcommand{\Cat}{\catname{Cat}}
\newcommand{\Psh}{\catname{Psh}}
\newcommand{\twoCat}{\catname{2-Cat}}
\newcommand{\MndK}{\catname{Mnd}(\twoCatK)}
\newcommand{\EndoK}{\catname{Endo}(\twoCatK)}
\newcommand{\MndCat}{\catname{Mnd}(\Cat)}
\newcommand{\EndoCat}{\catname{Endo}(\Cat)}
\newcommand{\RefEndoK}{\catname{Ref}(\catname{Endo}(\twoCatK))}
\newcommand{\CatTwo}{\catname{2}}
\newcommand{\SubSet}{\catname{Subset}}
\newcommand{\pabove}{\sqsubset}
\newcommand*\conj[1]{\bar{#1}}
\newcommand{\defeq}{\stackrel{\text{def}}{\coloneqq}}
\newcommand{\defcolor}[1]{\mathcolor{blue}{#1}}
\newcommand{\arrowdot}[0]{\xrightarrow{\bullet}}
\newcommand{\catTwo}{\mathbbm{2}}
%\newcommand{\catBArr}[0]{\catname{B}^{\mathbbm{2}}}
\newcommand{\catBArr}[0]{\catBarr}
\newcommand{\pcite}[1]{\parencite{#1}}
\newcommand{\catA}[0]{\catname{A}}
\newcommand{\catB}[0]{\catname{B}}
\newcommand{\catBarr}[0]{\catname{B}^\rightarrow}
\newcommand{\FArr}[0]{F^\rightarrow}
\newcommand{\DeltaArr}[0]{\Delta_\rightarrow}
\newcommand{\catOne}[0]{\catname{1}}
\newcommand{\catC}[0]{\catname{C}}
\newcommand{\catD}[0]{\catname{D}}
\newcommand{\catE}[0]{\catname{E}}
\newcommand{\catF}[0]{\catname{F}}
\newcommand{\catG}[0]{\catname{G}}
\newcommand{\catK}[0]{\catname{K}}
\newcommand{\catP}[0]{\catname{P}}
\newcommand{\catQ}[0]{\catname{Q}}
\newcommand{\catR}[0]{\catname{R}}
\newcommand{\catT}[0]{\catname{T}}
\newcommand{\catX}[0]{\catname{X}}
\newcommand{\catY}[0]{\catname{Y}}
\newcommand{\twoCatK}[0]{\mathcal{K}}
\newcommand{\twoCatX}[0]{\mathcal{X}}
\newcommand{\RefK}[0]{\catname{Ref}(\twoCatK)}
\newcommand{\RefCat}[0]{\catname{Ref}(\Cat)}
\newcommand{\Adj}{\catname{Adj}}
\newcommand{\AdjK}{\catname{Adj}(\twoCatK)}
\newcommand{\AdjRefK}{\catname{Adj}(\RefK)}
\newcommand{\AdjCatOverB}{\catname{Adj}(\CatOverB)}
\newcommand{\ControlK}{\catname{Control}(\twoCatK)}

\newcommand{\PushRef}[0]{\catname{Push}}
\newcommand{\SectRef}[0]{\catname{Sect}}
\newcommand{\Ref}[0]{\catname{Ref}}
\newcommand{\basisfunctor}{basis}
\newcommand{\cover}{\parallel}
%\newcommand{\CatOverB}{\Cat \cover \catB}
\newcommand{\CatOverB}{\Cat/\!/\catB}
\newcommand{\BOverCat}{\catB/\!/\Cat}
\newcommand{\CatOverC}{\Cat/\!/\catC}
\newcommand{\COverCat}{\catC/\!/\Cat}
\newcommand{\POverCat}{\catP/\!/\Cat}
\newcommand{\prehension}{prehension }
\newcommand{\prehensionFunctor}[1]{\{#1\}}
\newcommand{\prehPrime}{preh }
\newcommand{\To}{\Rightarrow}
\newcommand{\from}{\leftarrow}
\newcommand{\KOverB}{\twoCatK/\!/B}



%\newcommand{\xto}[2]{\xrightarrow {\ifstrempty{#1}{}{[#1]}}{#2}}
\newcommand{\xto}[2]{\xrightarrow {\ifstrempty{#1}{}{#1}}{#2}}
%\newcommand{\cata}[1]{\widetilde{#1}}
\newcommand{\cata}[1]{\llparenthesis{#1}\rrparenthesis}

\newcommand{\falg}[0]{$F$-algebra }
\newcommand{\galg}[0]{$G$-algebra }


\newcommand{\composeH}{\cdot}
\newcommand{\composeV}{\circ}
\newcommand{\composeHHidden}{}
\newcommand{\composeVHidden}{\circ}
\newcommand{\compose}{ }
\newcommand{\refine}{\sqsubset}











%%% mathdefsGene.tex
%
\newcommand{\e}{\epsilon}
\newcommand{\ee}{\zeta}
\newcommand{\ec}[1]{\mathit{#1}}
\newcommand{\p}{p}
\newcommand{\s}{\sigma}
\newcommand{\D}{\Delta}
\newcommand{\ue}{\upsilon}

% Taken from Adam Lupu-Sax ....................................................
%%% derivatives
\newcommand{\deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\derivc}[3]{\left. \frac{d#1}{d#2}\right|_{#3}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdc}[3]{\left. \frac{\partial #1}{\partial #2}\right|_{#3}}

%%% Dirac notation
\newcommand{\bra}[1]{\left\langle #1\right|}
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\braket}[2]{\left\langle #1 \left|#2\right.\right\rangle}
\newcommand{\braOket}[3]{\left\langle #1\left|#2\right|#3\right\rangle}

% calligraphic letters in math.
\def\cal#1{\mathcal{#1}}


% Taken from M Haggerty ......................................................
\def\avg#1{\left< #1 \right>}
\def\abs#1{\left| #1 \right|}
\def\recip#1{\frac{1}{#1}}
\def\vhat#1{\hat{{\bf #1}}}
\def\smallfrac#1#2{{\textstyle\frac{#1}{#2}}}
\def\smallrecip#1{\smallfrac{1}{#1}}

% SPSmith's definitions ......................................................
\def\spshalf{{1\over{2}}}
\def\Orabi{\Omega_{\rm rabi}}
\def\btt#1{{\tt$\backslash$#1}}




% My own .....................................................................

%%% Equations
\def\schrod{Schroedinger's Equation}
\def\helm{Helmholtz Equation}


%%% Equation environments
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bean{\begin{mathletters}\begin{eqnarray}}
\def\eean{\end{eqnarray}\end{mathletters}}


%%% macros for Feb 2000 PRL
\newcommand{\tbox}[1]{\mbox{\tiny #1}}
\newcommand{\half}{\mbox{\small $\frac{1}{2}$}}
\newcommand{\pit}{\mbox{\small $\frac{\pi}{2}$}}
\newcommand{\sfrac}[1]{\mbox{\small $\frac{1}{#1}$}}
\newcommand{\mbf}[1]{{\mathbf #1}}
% hack to get APS's \text style to work ok:
\def\text{\tbox}

\newcommand{\mV}{{\mathsf{V}}}
\newcommand{\mL}{{\mathsf{L}}}
\newcommand{\mA}{{\mathsf{A}}}
\newcommand{\lB}{\lambda_{\tbox{B}}}  % de Broglie
\newcommand{\ofr}{{(\mbf{r})}}       % (r vec)
\def\ofkr{(k;\mbf{r})}			% (k;r vec)
\def\ofks{(k;\mbf{s})}			% (k;s vec)
\newcommand{\ofs}{{(\mbf{s})}}       % (s vec)
\def\xt{\mbf{x}^{\tbox T}}		% x^T vec

\def\ce{\tilde{C}_{\tbox E}}		% C_E
\def\cew{\tilde{C}_{\tbox E}(\omega)}		% C_E(w)
\def\ceqmw{\tilde{C}^{\tbox{qm}}_{\tbox E}(\omega)}	% C^qm_E(w)
\def\cewqm{\tilde{C}^{\tbox{qm}}_{\tbox E}}	% C^qm_E(w) no omega
\def\ceqm{C^{\tbox{qm}}_{\tbox E}}	% C^qm_E no tilde
\def\cw{\tilde{C}(\omega)}		% C(w)
\def\cfw{\tilde{C}_{\cal F}(\omega)}		% C_F(w)

\def\tcl{\tau_{\tbox{cl}}}		% tau cl
\def\tcol{\tau_{\tbox{col}}}		% tau col
\def\terg{t_{\tbox{erg}}}		% t_erg
\def\tbl{\tau_{\tbox{bl}}}		% tau bl
\def\theis{t_{\tbox{H}}}		% t_Heis

\def\area{\mathsf{A}_D}			% piston effective area A_D 
\def\ve{\nu_{\tbox{E}}}			% nu_E, noise intensity
\def\vewna{\nu_E^{\tbox{WNA}}}		% nu_E for WNA

\def\dxcqm{\delta x^{\tbox{qm}}_{\tbox c}}	% x to mix levels.

%% operators
\newcommand{\rop}{\hat{\mbf{r}}}	% vector valued operators
\newcommand{\pop}{\hat{\mbf{p}}}



\newcommand*{\LargerCdot}{\raisebox{-0.25ex}{\scalebox{2}{$\cdot$}}}


\newcommand{\adjunction}[4]{#1 \underset{#4}{\stackrel{#3}{\rightleftharpoons}} #2}
\newcommand\functor[1][l]{\csname#1functor\endcsname}
\newcommand\lfunctor[4]{%
  \setbox0=\hbox{$#2$}%
  \kern\wd0%
  \ensurestackMath{\Centerstack[c]{#1\\ #2\\ \mathllap{#3\;\,}\mathclap{\DownArrow}\\#4}}%
}
\newcommand\rfunctor[4]{%
  \setbox0=\hbox{$#2$}%
  \ensurestackMath{\Centerstack[c]{#1 \\ #2\\ \mathclap{\DownArrow} \mathrlap{\,\;#3}\\#4}}%
  \kern\wd0%
}
\newcommand\lrfunctor[5]{%
  \setbox0=\hbox{$#2$}%
  \ensurestackMath{\Centerstack[c]{#1 \\ #2\\ \mathllap{#3\;\,} \mathclap{\DownArrow} \mathrlap{\,\;#4}\\#5}}%
  \kern\wd0%
}
\newcommand\functormapsto[1]{\mathrel{\ensurestackMath{\Centerstack[c]{\xrightarrow{\qquad #1 \qquad} \\ \longmapsto\\ \longmapsto \\\longmapsto}}}}
\setstackgap{L}{1.3\normalbaselineskip}
\stackMath


\newcommand\reallywidecheck[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern-0.0pt\bigwedge\kern-0.0pt}%
    {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
  }{\textheight}% 
}{0.5ex}}%
\stackon[1pt]{#1}{\scalebox{-1}{\tmpbox}}%
}



